Psycholinguistics meets Continual Learning: Measuring Catastrophic Forgetting in Visual Question Answering

We study the issue of catastrophic forgetting in the context of neural multimodal approaches to Visual Question Answering (VQA). Motivated by evidence from psycholinguistics, we devise a set of linguistically-informed VQA tasks, which differ by the types of questions involved (Wh-questions and polar questions). We test what impact task difficulty has on continual learning, and whether the order in which a child acquires question types facilitates computational models. Our results show that dramatic forgetting is at play and that task difficulty and order matter. Two well-known current continual learning methods mitigate the problem only to a limiting degree.

==> analysis.tex <==
\section{Further Analysis and Discussion}
\label{sec:analysis}


 
%--------------------------
\paragraph{Error analysis} 
%--------------------------
We looked into the confusion matrices produced by the models on the
two testa sets. The LSTM-CNN-SA model which has been trained on the
wh-questions never does mistakes across the attributes, it always
confuses labels within the same attribute type e.g., a color with a
color. The Cumulative model never gives the wrong answer type
(answering as yes/no question with an attribute or viceversa a
wh-question with a yes/no.) whereas the Naive models does this kind of
mistakes a lot: it almost always answers with the labels of the task
B, questions of the task A. The \emph{EWC} does better than the Naive
baseline: in the {\sc wh-to-yes/no} setting, it answers with an
attribute of the correct class almost all the wh question about color
and shapes, whereas it answers to all the wh questions about size and
to almost all those about material with a yes/no answer; instead in
the {\sc yes/no-to-wh} setting, it answers all the yes/no questions
with an attribute, quite often but not always, it gives the attribute
of the class on which the yes/no question is about (e.g., ``Does the
object on the left has the same color $\ldots$'' is answer with a
color). Interestingly, the \emph{Reharsal} model almost never confuses
the question type in both settings.  In the {\sc Wh-to-Yes/No}
setting, it only answers with yes/no 2 wh questions about size, and it
makes a few confusions across attributes, e.g. 8 times it answers with
a size a question about color; in the {\sc yes/no-to-wh} setting it
answer with attributes only 1 yes/no question about shape and 1 about size.

%We looked into the confusion matrices produced by the models on the
%%two sample test set. The LSTM-CNN-SA model which has been trained on
%the wh-questions does not guess the type of the answer of the yes/no
%question correctly, \rf{I don't understand which model this is - which
  %oder {\sc wh$\rightarrow$y/n} or {\sc y/n$\rightarrow$wh}? which CL
 % method? RB: no ORDER. It's the LSTM-CNN-SA trained on wh and tested
 % on the sample test set that contains both wh and yes/no} it answers
%them with an attribute, but quite often it gives the attribute which
%is the focus of the question. For instances, if the question is asking
%to compare the material of two objects like in Figure~\ref{fig:tasks},
%``Does the cyan ball have the same material \ldots?'', the model
%answers with one of the possible material.  When it confuses the
%attribute it self, quite often it answers with one of the ``size''
%possibilities even though the question is asking to compare the color,
%the shape or the material of the objects.  Interestingly, when tested
%on task A after having been exposed to TASK B, the \emph{Reharsal}%
%model never confuses \emph{the question type}, e.g., it never answers
%with a yes/no-answer a wh-question. Instead the \emph{EWC} does so
%238/1024 times when the task to be remembered are the wh-questions,
%and always when they are the yes/no-questions.}


\paragraph{Multimodal Representations}
To further analyse the results, we zoom into two samples of the wh and
yes/no test sets, each containing 512 questions. To visualize how the
continual learning methods effect how the model grounds the questions
into vision, we inspectioned the penultimate hidden layer of the
models produced by giving as input the two sample test
sets. Figure~\ref{fig:clusters} reports the clusters obtained from
these layers for each model. As we can see, the model trained on
wh-questions (up left corner) can discriminate the wh-questions about
color, material and shape quite well, it clusters the yes/no questions
together with the query-size independently on which is the attribute
on which the question focuses on; whereas the model trained on
yes/no-questions (up right corner) has very confused representations.
The other images in Figure~\ref{fig:clusters} show how the LSTM-CNN-SA
model trained on Wh changes its multimodal representation when it sees
also the yes/no questions. 
The cumulative (middle right) images is quite interesting, it shows
that the model can discriminate quite well all the eight types of
sub-questions and that the yes/no ones are closer to each other than
the wh-questions. This could be behind the higher difficulties the
models encounter in answering them. The Reharsal model remebers pretty
well how to discriminate the wh-questions on the base of their focused
attribute, whereas has a rather confused representation of the yes/no
questions. The EWC instead clusters most of the yes/no questions close
to the wh-questions about size.

\begin{figure*}
\begin{tabular}{c cc}
& Wh & Yes/No\\
\rotatebox{90}{LSTM-CNN-SA} & \includegraphics[width=0.5\linewidth]{img/model-A.png}
 &\includegraphics[width=0.5\linewidth]{img/model-B.png}\\[2mm]
 & Naive  & Cumulative\\
\rotatebox{90}{\sc Wh-to-Yes/No} & \includegraphics[width=0.5\linewidth]{img/model-finetuned-B.png}
 &\includegraphics[width=0.5\linewidth]{img/model-cumulative.png}\\[2mm]
& Reharsal   & EWC   \\
\rotatebox{90}{\sc Wh-to-Yes/No} & \includegraphics[width=0.5\linewidth]{img/model-reharsal.png}
 &\includegraphics[width=0.5\linewidth]{img/model-ewc.png}\\
\end{tabular}\caption{Analysis of the penultime hidden layer. \textbf{Up}: Model trained on wh-q (left)
  vs.\ Model trained on Yes/No-q (right). \textbf{Middle}: Model
  trained on Wh- and fine-tuned on Yes/No-questions (left) vs.\ Model trained
  cumulatively on Wh- and Yes/No-questions (right). \textbf{Down}: Model
  reharsed on Wh- while being trained on Yes/No-questions (left)
  vs.\ EWC model trained on Yes/No after having being trained on Wh (right).}\label{fig:clusters}
\end{figure*}

\cut{We have looked into the confusion matrices of the models. They almost
never confuse the question type (wh vs yes/no) or the attribute (for
the wh-questions) of the B task. Hence, their mistakes are always within a certain
attribute class. The only model that shows some confusion accross the
question types is the EWC model, after having been trained first on
wh- and then on yes/no questions it confuse several wh- as yes/no
questions~\ref{tab:confusion}. The Nive model that forget completely
the task A confuses the
question type completely, whereas this does not happen with the
Reharsal model, as shown in Table~\ref{tab:confusion} (down).

\begin{table*}
\centering
\begin{tabular}{cc}
\includegraphics[width=0.75\linewidth]{img/confusion-matrices-wh.png}\\
\includegraphics[width=0.75\linewidth]{img/confusion-reharsal-wh.png}
\end{tabular}\caption{NON-BALANCED:Confusion Matrix of the EWC (up) and the
Reharsal model (down)} \label{tab:confusion}
\end{table*}
}



